Properties of the Youngest Protostars in Perseus, Serpens, and Ophiuchus

We present an unbiased census of deeply embedded protostars in Perseus, Serpens, and Ophiuchus, assembled by combining large-scale 1.1 mm Bolocam continuum and Spitzer Legacy surveys. We identify protostellar candidates based on their mid-infrared properties, correlate their positions with 1.1 mm core positions, and construct well-sampled SEDs using our extensive wavelength coverage (lam=1.25-1100 micron). Source classification based on the bolometric temperature yields a total of 39 Class 0 and 89 Class I sources in the three cloud sample. We compare to protostellar evolutionary models using the bolometric temperature-luminosity diagram, finding a population of low luminosity Class I sources that are inconsistent with constant or monotonically decreasing mass accretion rates. This result argues strongly for episodic accretion during the Class I phase, with more than 50% of sources in a ``sub-Shu'' (dM/dt < 1e-6 Msun/yr) accretion state. Average spectra are compared to protostellar radiative transfer models, which match the observed spectra fairly well in Stage 0, but predict too much near-IR and too little mid-IR flux in Stage I. Finally, the relative number of Class 0 and Class I sources are used to estimate the lifetime of the Class 0 phase; the three cloud average yields a Class 0 lifetime of 1.7e5 yr, ruling out an extremely rapid early accretion phase. Correcting photometry for extinction results in a somewhat shorter lifetime (1.1e5 yr). In Ophiuchus, however, we find very few Class 0 sources (N(Class0)/N(ClassI)=0.1-0.2), similar to previous studies of that cloud. The observations suggest a consistent picture of nearly constant average accretion rate through the entire embedded phase, with accretion becoming episodic by at least the Class I stage, and possibly earlier.

==> tab2.tex <==
\ProvidesFile{tab1.tex}
\renewcommand{\thefootnote}{\alph{footnote}}
%\scriptsize
\vspace{1in}
\begin{center}
\begin{longtable*}{llccccll}
%\tablecolumns{8}
%\tablewidth{0pc}
\caption[]{\\ Bolometric temperatures, luminosities, and envelope masses of embedded protostars in Perseus} \label{boltabp} \\
\hline \hline \\[-2ex]
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{c2d name/position} &
\multicolumn{1}{c}{$\mathrm{T_{bol}}$} & \multicolumn{1}{c}{$\mathrm{L_{bol}}$} &
\multicolumn{1}{c}{$\alpha_{\mathrm{IR}}$} & \multicolumn{1}{c}{$\mathrm{M_{env}}$} &
\multicolumn{1}{c}{Bolocam ID} & \multicolumn{1}{c}{Other Names} \\[0.5ex]
\multicolumn{1}{c}{} & \multicolumn{1}{c}{(SSTc2dJ...)} &
\multicolumn{1}{c}{(K)} & \multicolumn{1}{c}{($\mathrm{L}_{\sun}$)} &
\multicolumn{1}{c}{} & \multicolumn{1}{c}{$\mathrm{M}_{\sun}$)} &
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\[0.5ex] \hline \\[-1.8ex]
\endfirsthead
\\[1in]
\multicolumn{7}{c}{{\tablename} \thetable{} -- Continued} \\[0.5ex]
\hline \hline \\[-2ex]
\multicolumn{1}{c}{ID} & \multicolumn{1}{c}{c2d name/position} &
\multicolumn{1}{c}{$\mathrm{T_{bol}}$} & \multicolumn{1}{c}{$\mathrm{L_{bol}}$} &
\multicolumn{1}{c}{$\alpha_{\mathrm{IR}}$} & \multicolumn{1}{c}{$\mathrm{M_{env}}$} &
\multicolumn{1}{c}{Bolocam ID} & \multicolumn{1}{c}{Other Names} \\[0.5ex] 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{(SSTc2dJ...)} &
\multicolumn{1}{c}{(K)} & \multicolumn{1}{c}{($\mathrm{L}_{\sun}$)} &
\multicolumn{1}{c}{} & \multicolumn{1}{c}{$\mathrm{M}_{\sun}$)} &
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\[0.5ex] \hline \\[-1.8ex]
\endhead

%\multicolumn{7}{l}{{Continued on Next Page\ldots}} \\
\endfoot

\\[-1.8ex] \hline \hline
\endlastfoot

%\startdata
\hline
\multicolumn{7}{c}{Class 0}  \\
\hline
Per-emb 1  &  J034356.53+320052.9   &  24 (5)  &  1.5 (0.4)  &  0.5 (0.18)  &  3.02 (0.08)  &  Bolo 103  &  \object{HH 211}  \\ 
Per-emb 2  &  J033217.95+304947.6   &  25 (2)  &  1.3 (0.2)  &  1.07 (0.11)  &  2.88 (0.08)  &  Bolo 66  & \object{IRAS 03292+3039} \\ 
Per-emb 3  &  J032900.52+311200.7   &  30 (4)  &  0.69 (0.15)  &  2.16 (0.1)  &  0.29 (0.03)  &  Bolo 41  &   \\  %JJK2007 18
Per-emb 4  &  J032839.10+310601.8   &  31 (3)  &  0.22 (0.03)  &  1.68 (0.06)  &  0.36 (0.02)  &  Bolo 30  \\  %JJK2007 12
Per-emb 5  &  J033120.96+304530.2   &  33 (1)  &  1.2 (0.2)  &  0.98 (0.06)  &  0.95 (0.04)  &  Bolo 65  &  \object{IRAS 03282+3035} \\ 
Per-emb 6  &  J033314.40+310710.9   &  36 (5)  &  0.64 (0.01)  &  2.22 (0.06)  &  1.04 (0.1)  &  Bolo 79\tablenotemark{a} &  \\ %\object[\[HKM99\] B1-d]{B1-d} \\ 
Per-emb 7  &  J033032.68+302626.5   &  37 (4)  &  0.15 (0.06)  &  2.08 (0.07)  &  0.99 (0.08)  &  Bolo 62 &  \\ 
Per-emb 8  &  J034443.94+320136.1   &  40 (6)  &  3.0 (0.5)  &  0.96 (0.07)  &  0.63 (0.06)  &  Bolo 116\tablenotemark{a}  &  \\ 
Per-emb 9  &  J032951.82+313906.1   &  41 (2)  &  0.46 (0.01)  &  3.44 (0.11)  &  0.64 (0.04)  &  Bolo 59  &  \object{IRAS 03267+3128} \\  
Per-emb 10  &  J033316.45+310652.5   &  47 (14)  &  0.27 (0.66)  &  1.73 (0.09)  &  1.57 (0.16)  &  Bolo 79\tablenotemark{a}  & \\  % JJK2007 35
Per-emb 11  &  J034356.85+320304.6   &  49 (15)  &  0.45 (0.85)  &  1.37 (0.09)  &  1.78 (0.04)  &  Bolo 104 &  \object[NAME IC 348 MMS]{IC 348-MMS} \\ 
Per-emb 12  &  J032910.50+311331.0   &  51 (17)  &  4.2 (4.4)  &  2.58 (0.08)  &  7.75 (0.78)  &  Bolo 48\tablenotemark{a}  &  \object[\[JCC87\] IRAS 4A1]{NGC 1333-IRAS 4A} \\ 
Per-emb 13  &  J032912.04+311301.5   &  54 (18)  &  1.6 (2.0)  &  0.55 (0.06)  &  3.66 (0.37)  &  Bolo 48\tablenotemark{a}  &  \object[\[JCC87\] IRAS 4B]{NGC 1333-IRAS 4B} \\ 
Per-emb 14  &  J032913.52+311358.0   &  54 (14)  &  0.49 (0.32)  &  2.41 (0.13)  &  0.5 (0.05)  &  Bolo 48\tablenotemark{a} &  \object[\[JCC87\] IRAS 4C]{NGC 1333-IRAS 4C} \\ 
Per-emb 15  &  J032904.05+311446.6   &  56 (16)  &  0.53 (0.67)  &  1.43 (0.06)  &  1.16 (0.12)  &  Bolo 46  & \\
Per-emb 16  &  J034350.95+320324.8   &  56 (17)  &  0.38 (0.62)  &  1.51 (0.06)  &  1.15 (0.11)  &  Bolo 102\tablenotemark{a}  & \\ % JJK2007 41
Per-emb 17  &  J032739.09+301303.0   &  59 (11)  &  4.2 (0.1)  &  2.68 (0.06)  &  0.51 (0.03)  &  Bolo 22 & \object[IRAS 03245+3002]{RNO 15-FIR}  \\ 
Per-emb 18  &  J032911.25+311831.3   &  59 (12)  &  2.8 (1.7)  &  1.94 (0.06)  &  2.47 (0.07)  &  Bolo 49\tablenotemark{b}  & \\  % JJK2007 24
Per-emb 19  &  J032923.49+313329.5   &  60 (3)  &  0.36 (0.05)  &  1.51 (0.06)  &  0.64 (0.05)  &  Bolo 57 & \\  %\object[\[LMG94\] Per 4]
Per-emb 20  &  J032743.23+301228.8   &  60 (14)  &  1.7 (0.01)  &  2.39 (0.06)  &  0.5 (0.03)  &  Bolo 23  &  \object[NAME LDN l1455 IRS 4]{L1455-IRS 4} \\
Per-emb 21  &  J032910.68+311820.5   &  63 (12)  &  2.8 (1.9)  &  1.95 (0.06)  &  2.47 (0.07)  &  Bolo 49\tablenotemark{b}  & \\  % JJK2007 23
Per-emb 22  &  J032522.33+304514.0   &  63 (11)  &  1.7 (1.1)  &  2.34 (0.07)  &  1.41 (0.14)  &  Bolo 5  & \object[IRAS 03222+3034]{L 1448-IRS2}   \\ 
Per-emb 23  &  J032917.16+312746.4   &  66 (18)  &  0.29 (0.33)  &  1.75 (0.06)  &  0.5 (0.05)  &  Bolo 52  &  \\ % JJK2007 27
Per-emb 24  &  J032845.30+310542.0   &  67 (10)  &  0.43 (0.01)  &  1.11 (0.05)  &  0.19 (0.02)  &  Bolo 33\tablenotemark{a}  &  \\[1in] 
Per-emb 25  &  J032637.46+301528.0   &  68 (12)  &  0.95 (0.02)  &  1.09 (0.05)  &  0.5 (0.08)  &  Bolo 18  &  \\ %\object{IRAS 03235+3004} \\ 
Per-emb 26  &  J032538.82+304406.3   &  69 (7)  &  4.4 (1.5)  &  2.16 (0.06)  &  1.87 (0.19)  &  Bolo 10\tablenotemark{a}  & \object[LDN 1448C]{L 1448-C}  \\ 
Per-emb 27\tablenotemark{c}  &  J032855.56+311436.6   &  69 (1)  &  19.0 (0.4)  &  3.03 (0.12)  &  2.81 (0.28)  &  Bolo 38\tablenotemark{a}  &  \object[\[JCC87\] IRAS 2A]{NGC 1333-IRAS 2A}  \\ 
\hline
\multicolumn{7}{c}{Class I} \\
\hline
Per-emb 28  &  J034351.02+320307.9   &  72 (25)  &  0.28 (0.37)  &  -0.28 (0.06)  &  0.62 (0.06)  &  Bolo 102\tablenotemark{a}  & \\ % JJK2007 42
Per-emb 29  &  J033317.85+310932.0   &  76 (20)  &  1.8 (2.5)  &  3.33 (0.06)  &  3.84 (0.09)  &  Bolo 80  & \object[\[HKM99\] B1-c]{B1-c} \\ 
Per-emb 30  &  J033327.28+310710.2   &  78 (6)  &  1.7 (0.01)  &  1.93 (0.05)  &  0.59 (0.06)  &  Bolo 84  &  \\  % JJK2007 40
Per-emb 31  &  J032832.55+311105.2   &  80 (13)  &  0.16 (0.01)  &  0.78 (0.05)  &  0.19 (0.02)  &  Bolo 25  & \\ % JJK2007 9
Per-emb 32  &  J034402.40+320204.9   &  84 (29)  &  0.16 (0.31)  &  1.53 (0.06)  &  0.63 (0.02)  &  Bolo 106  & \\ % JJK2007 32
Per-emb 33  &  J032536.48+304522.3   &  90 (18)  &  4.3 (3.7)  &  2.62 (0.07)  &  4.47 (0.45)  &  Bolo 8 & \object[LDN 1448N]{L 1448-N}  \\ 
Per-emb 34  &  J033015.12+302349.2   &  99 (13)  &  1.6 (0.1)  &  1.7 (0.05)  &  0.46 (0.07)  &  Bolo 60 & \object[IRAS 03271+3013]{IRAS 03271+3013}  \\ 
Per-emb 35  &  J032837.09+311330.7   &  103 (26)  &  9.1 (0.3)  &  2.35 (0.08)  &  0.44 (0.04)  &  Bolo 29 & \object[IRAS 03255+3103]{NGC 1333-IRAS 1}  \\ 
Per-emb 36  &  J032857.36+311415.7   &  106 (12)  &  5.3 (1.0)  &  1.6 (0.06)  &  0.74 (0.07)  &  Bolo 38\tablenotemark{a} &  \\ %NGC 1333-IRAS 2B (6,9)  \\ 
Per-emb 37  &  J032918.27+312320.0   &  106 (21)  &  0.07 (0.35)  &  1.26 (0.06)  &  0.44 (0.04)  &  Bolo 54\tablenotemark{a} & \\ % JJK2007 28
Per-emb 38  &  J033229.18+310240.9   &  115 (21)  &  0.54 (0.01)  &  0.4 (0.05)  &  0.45 (0.08)  &  Bolo 68  & \\ 
Per-emb 39  &  J033313.78+312005.2   &  125 (47)  &  0.04 (0.08)  &  1.44 (0.06)  &  0.41 (0.04)  &  Bolo 78  &  \\  % JJK2007 34
Per-emb 40  &  J033316.66+310755.2   &  132 (25)  &  1.5 (1.0)  &  1.57 (0.05)  &  1.12 (0.11)  &  & \object[\[HKM99\] B1-a]{B1-a} \\ 
Per-emb 41  &  J033320.30+310721.3   &  157 (72)  &  0.17 (0.36)  &  0.88 (0.05)  &  1.5 (0.15)  &  Bolo 81  & \object[\[HKM99\] B1-b]{B1-b} \\ 
Per-emb 42  &  J032539.10+304358.0   &  163 (51)  &  0.68 (0.85)  &  2.36 (0.06)  &  1.82 (0.18)  &  Bolo 10\tablenotemark{a} & \\ % l1448C ?
Per-emb 43  &  J034202.16+314802.1   &  176 (42)  &  0.07 (0.06)  &  1.47 (0.05)  &  0.07 (0.02)  &  &  \\ 
Per-emb 44\tablenotemark{c}  &  J032903.76+311603.7   &  188 (9)  &  32.5 (7.1)  &  1.21 (0.08)  &  3.25 (0.32)  &  Bolo 43 &  \object[\[SVS76\] NGC 1333 13A]{SVS 13A}  \\ 
Per-emb 45  &  J033309.57+310531.2   &  197 (93)  &  0.05 (0.06)  &  1.13 (0.05)  &  0.21 (0.02)  &  &  \\ 
Per-emb 46  &  J032800.40+300801.3   &  221 (7)  &  0.3 (0.07)  &  0.95 (0.05)  &  0.17 (0.02)  &  &  \\ 
Per-emb 47  &  J032834.50+310051.1   &  230 (17)  &  1.2 (0.1)  &  0.83 (0.05)  &  0.12 (0.02)  &  & \object{IRAS 03254+3050} \\ 
Per-emb 48  &  J032738.23+301358.8   &  238 (14)  &  0.87 (0.04)  &  -0.19 (0.05)  &  0.34 (0.04)  &  Bolo 21 &  \object[\[TPB97\] L 1455 FIR 2]{L1455 FIR2} \\ 
Per-emb 49  &  J032912.94+311814.4   &  239 (68)  &  1.1 (0.7)  &  1.05 (0.05)  &  0.77 (0.08)  &  Bolo 49\tablenotemark{a} & \object{ASR 30} \\ 
Per-emb 50\tablenotemark{d}  &  J032907.76+312157.2   &  254 (23)  &  10.0 (3.0)  &  2.18 (0.1)  &  1.62 (0.16)  &  Bolo 47 & \\ 
Per-emb 51  &  J032834.53+310705.5   &  263 (115)  &  0.07 (0.1)  &  0.54 (0.05)  &  0.24 (0.04)  &  Bolo 28 & \\ % JJK2007 10
Per-emb 52  &  J032839.72+311731.9   &  278 (119)  &  0.16 (0.21)  &  0.57 (0.05)  &  0.49 (0.05)  &  Bolo 31\tablenotemark{a} & \\ 
Per-emb 53  &  J034741.56+325143.9   &  287 (8)  &  4.7 (0.9)  &  0.78 (0.05)  &  1.67 (0.08)  &  Bolo 122 & \object[NAME BARN 5 IRS 1]{B5-IRS1}  \\ 
Per-emb 54\tablenotemark{d}  &  J032901.57+312020.7   &  304 (63)  &  6.2 (2.6)  &  2.09 (0.08)  &  1.87 (0.19)  &  Bolo 42 &  \object[ASR 114]{NGC 1333-IRAS 6} \\ 
Per-emb 55  &  J034443.33+320131.4   &  309 (64)  &  1.8 (0.8)  &  0.5 (0.05)  &  0.32 (0.03)  &  Bolo 116\tablenotemark{a} & \object{IRAS 03415+3152} \\ 
Per-emb 56  &  J034705.42+324308.4   &  312 (1)  &  0.54 (0.09)  &  0.36 (0.05)  &  0.14 (0.02)  &   &  \object{IRAS 03439+3233} \\ 
Per-emb 57  &  J032903.33+312314.6   &  313 (200)  &  0.09 (0.45)  &  1.13 (0.05)  &  0.11 (0.02)  &   &  \\ 
Per-emb 58  &  J032858.44+312217.4   &  322 (88)  &  0.63 (0.47)  &  0.83 (0.05)  &  0.71 (0.07)  &  Bolo 40  & \\ 
Per-emb 59  &  J032835.04+302009.9   &  341 (179)  &  0.04 (0.06)  &  0.15 (0.05)  &  0.14 (0.02)  &  Bolo 27  & \\ 
Per-emb 60  &  J032920.07+312407.5   &  363 (240)  &  0.28 (1.05)  &  0.42 (0.05)  &  0.52 (0.05)  &  Bolo 54\tablenotemark{a}  & \\ 
Per-emb 61  &  J034421.33+315932.6   &  371 (107)  &  0.24 (0.16)  &  0.21 (0.05)  &  0.17 (0.02)  &  Bolo 113  & \\ 
Per-emb 62  &  J034412.98+320135.4   &  378 (29)  &  1.8 (0.4)  &  0.37 (0.05)  &  0.12 (0.02)  &  &  \\ 
Per-emb 63  &  J032843.28+311733.0   &  436 (9)  &  1.9 (0.4)  &  0.36 (0.05)  &  0.25 (0.02)  &  Bolo 31\tablenotemark{a}  & \\ 
Per-emb 64  &  J033312.85+312124.1   &  438 (8)  &  3.2 (0.6)  &  0.41 (0.05)  &  0.53 (0.07)  &  Bolo 76  & \\ 
Per-emb 65  &  J032856.31+312227.8   &  440 (191)  &  0.16 (0.16)  &  -0.14 (0.05)  &  0.25 (0.02)  &   & \\ 
Per-emb 66  &  J034345.15+320358.6   &  542 (110)  &  0.69 (0.22)  &  -0.22 (0.05)  &  0.24 (0.02)  &   &
%\enddata
%\clearpage
%\footnotetext{
\footnotetext{NOTE -- The envelope mass $M_{env}$ is calculated from the 1.1~mm flux assuming a dust temperature $T_D = 15$~K.  
Bolocam IDs are from Papers I--III, and indicate that the protostellar source is within 1.0 core FWHM of a given Bolocam core. If no ID is listed, the source was not originally identified as a distinct 1.1~mm core, but there is detectable ($\gtrsim3\sigma$) 1.1~mm emission at the position of the source.
Uncertianties for $T_{bol}$, $L_{bol}$, and $M_{env}$ are given in parentheses; uncertainties for $T_{bol}$ and $L_{bol}$ are taken to be the difference of values calculated by the midpoint and prismoidal methods (see \S\ref{appendsect}).  Uncertainties in $M_{env}$ are from the photometric errors in the total flux only.  Absolute uncertainties in the mass may be a factor of 2 or more, from uncertainties in $d$, $\kappa_{1mm}$ and $T_D$, but relative values should be much more accurate.} 
%\vspace{-4in}
\footnotetext[1]{More than one protostar is associated with this Bolocam core or source is in a crowded region; mass is based on flux measured in a $30-40\arcsec$ diameter aperature.}
\footnotetext[2]{More than one protostar is associated with this Bolocam core; mass is based on dividing Bolocam core flux equally (source separation is less than 30$\arcsec$).}
\footnotetext[3]{Saturated $24\micron$ flux has been replaced with IRAS $25\micron$ flux for the calculation of \lbol\ and \tbol.}
\footnotetext[4]{Saturated at either $24\micron$ or $70\micron$ so \lbol\ is likely an underestimate, but the IRAS beam is too confused to measure reliable $25\micron$ or $60\micron$ fluxes.}
\end{longtable*}
\end{center}
\normalsize

\renewcommand{\thefootnote}{\arabic{footnote}}

\endinput


==> tab3.tex <==
\ProvidesFile{tab2.tex}
\begin{deluxetable*}{llccccll}[!ht]
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Bolometric temperatures, luminosities, and envelope masses of cold protostars in Serpens\label{boltabs}}
\tablehead{
\colhead{ID} & \colhead{c2d name/position} & \colhead{$\mathrm{T_{bol}}$} & \colhead{$\mathrm{L_{bol}}$} & \colhead{$\alpha_{\mathrm{IR}}$} & \colhead{$\mathrm{M_{env}}$} & \colhead{Bolocam ID} & \colhead{Other Names} \\
\colhead{} & \colhead{(SSTc2dJ...)} & \colhead{(K)} & \colhead{($\mathrm{L}_{\sun}$)} & \colhead{} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{} & \colhead{}
}
\startdata
\hline
\multicolumn{7}{c}{Class 0} \\
\hline
Ser-emb 1  &  J182909.24+003132.3   &  39 (2)  &  1.6 (0.1)  &  2.27 (0.08)  &  1.16 (0.02)  &  Bolo 15  & \\ 
Ser-emb 2  &  J182952.44+003611.7   &  42 (10)  &  1.0 (0.1)  &  0.77 (0.05)  &  0.54 (0.03)  &  Bolo 24\tablenotemark{a} &  \\ %IRAS 18273+0034  \\ 
Ser-emb 3  &  J182854.84+002952.5   &  51 (12)  &  2.6 (0.1)  &  1.91 (0.06)  &  1.54 (0.15)  &  Bolo 8\tablenotemark{a}  &  \\ %IRAS 18263+0027 \\ 
Ser-emb 4  &  J183000.72+011301.4   &  54 (16)  &  1.2 (1.6)  &  1.68 (0.08)  &  2.56 (0.03)  &  Bolo 28\tablenotemark{a}  &  \\ 
Ser-emb 5  &  J182854.84+001832.6   &  56 (12)  &  0.16 (0.1)  &  0.9 (0.06)  &  0.24 (0.02)  &  Bolo 7\tablenotemark{a}  & \\ 
Ser-emb 6  &  J182949.56+011521.9   &  56 (12)  &  11.0 (6.0)  &  2.65 (0.07)  &  7.98 (0.07)  &  Bolo 23\tablenotemark{a} & \object[NAME S68 FIR]{FIRS1}  \\ %FIRS 1 
Ser-emb 7  &  J182854.12+002929.9   &  58 (13)  &  3.1 (0.1)  &  1.36 (0.06)  &  1.67 (0.17)  &  Bolo 8\tablenotemark{a}  & \\ %IRAS 18263+0027 
Ser-emb 8\tablenotemark{b}  &  J182948.12+011644.9   &  58 (16)  &  2.1 (2.4)  &  1.37 (0.06)  &  3.72 (0.37)  &  Bolo 22\tablenotemark{a}  &  \object[SH 2-68 N]{S68N}  \\ 
%Ser-emb 9  &  J182959.28+011401.6   &  59 (16)  &  1.7 (1.6)  &  1.03 (0.1)  &  2.56 (0.04)  &  Bolo 26  & \\ 
Ser-emb 9  &  J182855.92+002944.7   &  66 (21)  &  0.34 (0.63)  &  1.89 (0.06)  &  1.19 (0.12)  &  Bolo 8\tablenotemark{a}  & \\ %IRAS 18263+0027 
\hline
\multicolumn{7}{c}{Class I} \\
\hline
Ser-emb 10\tablenotemark{c,d}  &  J182845.12+005203.5   &  75 (14)  &  1.09 (0.05)  &  1.33 (0.06)  &  0.29 (0.03)  &  Bolo 3\tablenotemark{a}  &  IRAS 1862+0050  \\
Ser-emb 11  &  J182906.72+003034.3   &  77 (12)  &  1.9 (1.2)  &  1.66 (0.06)  &  1.39 (0.14)  &  Bolo 14\tablenotemark{a}  & \\ %IRAS 18265+0028
Ser-emb 12\tablenotemark{b}  &  J182952.08+011547.8   &  85 (9)  &  2.6 (1.2)  &  1.54 (0.06)  &  1.23 (0.12)  &  Bolo 23\tablenotemark{a}  & \object[NAME Serpens SMM 10 IR]{SMM 10 IR} \\ 
Ser-emb 13  &  J182902.04+003120.6   &  86 (31)  &  0.05 (0.09)  &  0.24 (0.06)  &  0.17 (0.02)  &  &  \\ 
Ser-emb 14  &  J183005.40+004104.5   &  100 (32)  &  0.08 (0.1)  &  1.3 (0.07)  &  0.19 (0.02)  &   & \\ 
Ser-emb 15  &  J182954.24+003601.3   &  101 (43)  &  0.17 (0.27)  &  -0.18 (0.06)  &  0.48 (0.05)  &  Bolo 24\tablenotemark{a}  & \\ %IRAS 18273+0034  \\ 
Ser-emb 16\tablenotemark{d}  &  J182844.76+005125.7   &  110 (26)  &  0.04 (0.6)  &  1.07 (0.05)  &  0.24 (0.02)  &  Bolo 3\tablenotemark{a}  & \\ 
Ser-emb 17  &  J182906.36+003043.2   &  117 (21)  &  1.5 (1.3)  &  1.7 (0.06)  &  1.38 (0.14)  &  Bolo 14\tablenotemark{a}  &  \\ %IRAS 18265+0028
Ser-emb 18  &  J182952.80+011456.0   &  120 (15)  &  1.2 (0.8)  &  1.49 (0.05)  &  0.74 (0.07)  &  Bolo 23\tablenotemark{a} & \\ 
Ser-emb 19  &  J183000.00+011311.6   &  129 (29)  &  2.0 (1.9)  &  2.57 (0.06)  &  2.56 (0.03)  &  Bolo 28\tablenotemark{a}  & \\ 
Ser-emb 20\tablenotemark{b}  &  J182949.20+011619.8   &  131 (3)  &  4.4 (2.1)  &  3.8 (0.11)  &  1.53 (0.15)  &  Bolo 22\tablenotemark{a} &  \\ % FU Ori star?
Ser-emb 21  &  J182951.00+011640.6   &  141 (37)  &  1.7 (1.5)  &  1.04 (0.05)  &  1.84 (0.18)  &  Bolo 22\tablenotemark{a} &  \\ 
Ser-emb 22  &  J182957.48+011300.5   &  157 (39)  &  2.6 (2.2)  &  1.01 (0.05)  &  2.35 (0.24)  &  Bolo 25\tablenotemark{a} &  \\ 
Ser-emb 23  &  J182957.84+011251.4   &  190 (23)  &  3.1 (1.5)  &  0.67 (0.05)  &  1.06 (0.11)  &  Bolo 25\tablenotemark{a} &  \\ % S68 2
Ser-emb 24  &  J183000.00+011158.9   &  249 (64)  &  1.8 (1.2)  &  1.15 (0.05)  &  1.14 (0.11)  &  Bolo 29 &  \\ 
Ser-emb 25  &  J182851.24+001927.3   &  250 (106)  &  0.06 (0.07)  &  0.45 (0.05)  &  0.16 (0.02)  &  Bolo 7\tablenotemark{a}  & \\ 
Ser-emb 26  &  J182958.92+011426.2   &  303 (139)  &  0.62 (0.73)  &  0.46 (0.05)  &  2.0 (0.2)  &  Bolo 26\tablenotemark{a}  & \\  % GCNM 112
Ser-emb 27\tablenotemark{b}  &  J182956.76+011446.5   &  322 (25)  &  5.8 (1.7)  &  0.3 (0.05)  &  0.69 (0.07)  &    \\  % CoKu Ser G7
Ser-emb 28\tablenotemark{d}  &  J182844.04+005337.9   &  360 (244)  &  0.19 (1.5)  &  0.45 (0.05)  &  0.26 (0.03)  &  Bolo 2  & \\ 
Ser-emb 29  &  J183002.88+011228.2   &  374 (101)  &  2.2 (1.3)  &  0.21 (0.05)  &  1.32 (0.13)  &  Bolo 28\tablenotemark{a}  & \\  % GCNM 160
Ser-emb 30  &  J182957.84+011405.7   &  560 (85)  &  13.8 (4.2)  &  0.28 (0.09)  &  1.9 (0.19)  &  Bolo 26\tablenotemark{a}  &  IRAS 18274+0112 \\
Ser-emb 31  &  J182931.92+011842.9   &  430 (15)  &  5.3 (1.0)  &  0.26 (0.05)  &  2.12 (0.07)  &  Bolo 20  & \\ 
Ser-emb 32  &  J183005.76+003931.7   &  431 (207)  &  0.05 (0.07)  &  -0.39 (0.05)  &  0.2 (0.02)  &  Bolo 32  & \\ 
Ser-emb 33\tablenotemark{e}  &  J182916.08+001822.7   &  437 (10)  &  1.7 (0.2)  &  -0.07 (0.05)  &  0.54 (0.04)  &  Bolo 17 &  IRAS 18267+0016  \\
Ser-emb 34  &  J182902.76+003009.5   &  631 (410)  &  0.12 (0.28)  &  -0.14 (0.05)  &  0.22 (0.02)  &  Bolo 13  & \\ 
\enddata
\tablenotetext{a}{More than one protostar is associated with this Bolocam core or source is in a crowded region; mass is based on flux measured in a $30-40\arcsec$ diameter aperature.}
\tablenotetext{b}{Saturated at either $24\micron$ or $70\micron$ so \lbol\ is likely an underestimate, but the IRAS beam is too confused to measure reliable $25\micron$ or $60\micron$ fluxes.}
\tablenotetext{c}{Missing $70 \micron$ flux has been replaced with IRAS $60\micron$ flux for the calculation of \lbol\ and \tbol.}
\tablenotetext{d}{Source lies outside the $70 \micron$ map.}
\tablenotetext{e}{Saturated $24\micron$ flux has been replaced with IRAS $25\micron$ flux for the calculation of \lbol\ and \tbol.}
\tablecomments{Columns are as in Table~\ref{boltabp}, and uncertainties for $T_{bol}$, $L_{bol}$, and $M_{env}$ are given in parentheses.}
\end{deluxetable*}
\endinput


==> tab4.tex <==
\ProvidesFile{tab3.tex}
\begin{deluxetable*}{llccccll}[!ht]
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Bolometric temperatures, luminosities, and envelope masses of cold protostars in Ophiuchus\label{boltabo}}
\tablehead{
\colhead{ID} & \colhead{c2d name/position} & \colhead{$\mathrm{T_{bol}}$} & \colhead{$\mathrm{L_{bol}}$} & \colhead{$\alpha_{\mathrm{IR}}$} & \colhead{$\mathrm{M_{env}}$} & \colhead{Bolocam ID} & \colhead{Other Names}  \\
\colhead{} & \colhead{(SSTc2dJ...)} & \colhead{(K)} & \colhead{($\mathrm{L}_{\sun}$)} & \colhead{} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{} & \colhead{}
}
\startdata
\hline
\multicolumn{7}{c}{Class 0} \\
\hline
Oph-emb 1  &  J162821.72-243623.4   &  35 (2)  &  0.25 (0.01)  &  1.23 (0.06)  &  0.51 (0.04)  &  Bolo 26  & IRAS 16253-2429 \\ 
Oph-emb 2\tablenotemark{a}  &  J163222.56-242831.8   &  54 (8)  &  6.9 (1.2)  &  5.03 (0.2)  &  1.16 (0.02)  &  Bolo 36  & IRAS 16293-2422B \\ 
Oph-emb 3  &  J162625.80-242428.8   &  57 (10)  &  0.41 (0.15)  &  1.65 (0.07)  &  0.24 (0.02)  &  Bolo 9 & VLA 1623 (?) \\ %SM1 FIR2 (4) \\ 
\hline
\multicolumn{7}{c}{Class I} \\
\hline
Oph-emb 4  &  J163136.84-240419.9   &  77 (25)  &  0.18 (0.05)  &  -0.27 (0.05)  &  0.03 (0.01)  &    &  \\ 
Oph-emb 5  &  J162721.96-242727.7   &  87 (28)  &  0.08 (0.08)  &  -0.05 (0.05)  &  0.12 (0.01)  &  Bolo 17 &  \\ 
Oph-emb 6  &  J162705.40-243629.5   &  106 (14)  &  0.15 (0.09)  &  1.27 (0.05)  &  0.09 (0.01)  &  Bolo 14\tablenotemark{b}  &  LFAM26/GY197 \\ 
Oph-emb 7  &  J163151.96-245725.9   &  124 (39)  &  0.1 (0.13)  &  0.82 (0.05)  &  0.05 (0.01)  &  Bolo 33  & \\ 
Oph-emb 8\tablenotemark{c,d}  &  J162621.48-242304.2   &  133 (34)  &  18.3 (1.4)  &  1.46 (0.09)  &  0.22 (0.02)  &  Bolo 5  &  GSS 30 \\ 
Oph-emb 9  &  J162625.44-242301.3   &  135 (49)  &  0.1 (0.3)  &  0.87 (0.05)  &  0.53 (0.05)  &  Bolo 8  & GY 30  \\ 
Oph-emb 10  &  J163200.96-245642.7   &  145 (38)  &  2.7 (0.3)  &  1.39 (0.07)  &  0.05 (0.01)  &  Bolo 35  & L1689S/IRS67 \\ 
Oph-emb 11  &  J162717.64-242856.2   &  190 (1)  &  0.52 (0.06)  &  0.25 (0.05)  &  0.07 (0.01)  &   &  \\  % GY244
Oph-emb 12  &  J162724.48-244103.1   &  191 (30)  &  0.33 (0.16)  &  1.01 (0.05)  &  0.12 (0.01)  &  Bolo 18\tablenotemark{b} &  CRBR85 \\ 
Oph-emb 13\tablenotemark{c}  &  J162728.08-243933.4   &  193 (31)  &  7.2 (0.5)  &  2.29 (0.11)  &  0.11 (0.01)  &   & IRS 44/GY269 )\\ 
Oph-emb 14\tablenotemark{c}  &  J162727.00-244050.5   &  211 (7)  &  3.8 (0.7)  &  1.17 (0.08)  &  0.36 (0.04)  &  Bolo 18\tablenotemark{b} & IRS 43/GY265\\ 
Oph-emb 15  &  J163152.32-245536.1   &  240 (42)  &  0.13 (0.07)  &  1.07 (0.05)  &  0.08 (0.01)  &    & \\ 
Oph-emb 16\tablenotemark{c,d}  &  J162709.36-243718.4   &  257 (60)  &  17.9 (0.6)  &  1.69 (0.15)  &  0.07 (0.01)  &  Bolo 14\tablenotemark{b} & EL 29/GY214 \\ 
Oph-emb 17  &  J163135.76-240129.2   &  290 (18)  &  1.5 (0.1)  &  0.14 (0.05)  &  0.14 (0.02)  &  Bolo 30 &  IRAS 16295-2355 \\ 
Oph-emb 18  &  J162857.72-244054.8   &  304 (96)  &  0.03 (0.03)  &  0.67 (0.05)  &  0.04 (0.01)  &   & \\ 
Oph-emb 19  &  J162728.44-242720.8   &  309 (85)  &  0.47 (0.28)  &  -0.03 (0.05)  &  0.29 (0.03)  &  Bolo 20\tablenotemark{b} &  IRS45/GY273 \\ 
Oph-emb 20  &  J162706.84-243815.0   &  310 (23)  &  0.6 (0.16)  &  0.61 (0.05)  &  0.05 (0.01)  &  Bolo 13 & WL17/GY205 \\ 
Oph-emb 21\tablenotemark{c}  &  J162702.16-243727.1   &  331 (2)  &  5.2 (1.3)  &  1.53 (0.11)  &  0.08 (0.01)  &   &  WL16/GY182  \\ 
Oph-emb 22  &  J162640.56-242714.4   &  372 (160)  &  0.06 (0.09)  &  0.45 (0.05)  &  0.06 (0.01)  &   &  GY91/CRBR42 \\ 
Oph-emb 23  &  J162648.48-242838.6   &  428 (84)  &  0.12 (0.05)  &  0.02 (0.05)  &  0.03 (0.01)  &   &  WL2/GY128 \\ 
Oph-emb 24  &  J162737.08-244237.8   &  438 (87)  &  0.13 (0.06)  &  0.13 (0.05)  &  0.04 (0.01)  &   &  GY301 \\ 
Oph-emb 25  &  J163143.68-245524.6   &  496 (68)  &  0.28 (0.09)  &  0.23 (0.05)  &  0.04 (0.01)  &   & \\ % ISO-Oph 200 \\ 
Oph-emb 26  &  J162730.24-242743.2   &  528 (99)  &  0.93 (0.27)  &  -0.12 (0.05)  &  0.19 (0.02)  &  Bolo 20\tablenotemark{b}  &  IRS47/GY279 \\ 
Oph-emb 27  &  J162739.96-244314.8   &  551 (54)  &  0.74 (0.15)  &  -0.15 (0.05)  &  0.04 (0.01)  &  &   IRS51/GY315 \\ 
Oph-emb 28  &  J162721.60-244143.0   &  595 (57)  &  1.2 (0.2)  &  -0.03 (0.05)  &  0.04 (0.01)  &   &  IRS42/GY252 \\ 
\enddata
\tablenotetext{a}{Oph-emb 2 is saturated at $160\micron$; when the $100\micron$ IRAS flux is included the resulting \lbol\ is $16\pm6 \lsun$, consistent with the luminosity calculated by \citet{walker86} when scaled to a distance of 125~pc.}
\tablenotetext{b}{More than one protostar is associated with this Bolocam core or source is in a crowded region; mass is based on flux measured in a $30-40\arcsec$ diameter aperature.}
\tablenotetext{c}{Saturated $24\micron$ flux has been replaced with IRAS $25\micron$ flux for the calculation of \lbol\ and \tbol.}
\tablenotetext{d}{Saturated $70\micron$ flux has been replaced with IRAS $60\micron$ flux for the calculation of \lbol\ and \tbol.}
\tablecomments{Columns are as in Table~\ref{boltabp}, and uncertainties for $T_{bol}$, $L_{bol}$, and $M_{env}$ are given in parentheses.}
\end{deluxetable*}
\endinput


==> tab5.tex <==
\ProvidesFile{tab4.tex}
\begin{deluxetable*}{lccccll}[!ht]
%\tabletypesize{\footnotesize}
\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{Class~II sources detected at 1.1~mm in Perseus, Serpens, and Ophiuchus\label{cl2tab}}
\tablehead{
\colhead{c2d name/position } & \colhead{$\mathrm{T_{bol}}$ \ \ } & \colhead{$\mathrm{L_{bol}}$ \ \ } & \colhead{$\alpha_{\mathrm{IR}}$} & \colhead{$\mathrm{M_{1mm}}$\tablenotemark{a} \ \ } & \colhead{Bolocam ID\tablenotemark{b}} & \colhead{other names}  \\
\colhead{(SSTc2dJ...)} & \colhead{(K)} & \colhead{($\mathrm{L}_{\sun}$)} & \colhead{} & \colhead{($\mathrm{M}_{\sun}$)} & \colhead{} & \colhead{}
}
\startdata
\hline
\multicolumn{7}{c}{Perseus}  \\
\hline
J032747.66+301204.6  &  662 (15)  &  2.80 (0.05)   &  -0.09 (0.05)  &  0.82 (0.06)   &  Per-Bolo 24  &  RNO~15\tablenotemark{c} (1) \\ 
J034400.00+320154.1   &  700 (17)  &  1.60 (0.03)  &  -0.34 (0.05)  &  0.40 (0.04)   &  Per-Bolo 106$^{*}$ &  \\ 
J032900.00+312146.8   &  856 (26)  &  0.33 (0.01)  &  -0.83 (0.05)  &  0.90 (0.09)  &  Per-Bolo 40$^{*}$  &  LkH$\alpha$~353 (2)   \\ 
J034109.13+314438.0   &  873 (30)  &  1.70 (0.06)  &  -0.72 (0.05)  &  0.16 (0.02)   &  Per-Bolo 90  &   IRAS 03380+3135 \\ 
J032856.64+311835.6   &  993 (22)  &  0.42 (0.01)  &  -0.78 (0.05)  &  0.10 (0.02)  &  Per-Bolo 39$^{*}$  &   ASR~120 (3)  \\ 
J034548.27+322411.8   &  1096 (23)  &  5.00 (0.09) &  -0.72 (0.05)  &  0.10 (0.02)  &  Per-Bolo 120 &   LkH$\alpha$~330  (2) \\ 
J032917.66+312245.1   &  1297 (22)  &  1.50 (0.02) &  -0.77 (0.05)  &  0.19 (0.02)  &  Per-Bolo 54$^{*}$  &  LkH$\alpha$~270 (2)  \\ 
\hline
\multicolumn{7}{c}{Serpens}  \\
\hline
J182900.00+003003.1   &  806 (5)  &  0.19 (0.01)   &  -0.61 (0.05)  &  0.35 (0.03)   &  Ser-Bolo 13$^{*}$  &   \\ 
J183006.12+004233.9   &  871 (2)  &  3.60 (0.01)   &  -0.42 (0.05)  &  0.17 (0.01)    &  Ser-Bolo 33  &  \\ 
J182900.96+002931.6   &  892 (2)  &  1.20 (0.01)   &  -0.42 (0.05)  &  0.23 (0.02)    &  Ser-Bolo 13$^{*}$  &  \\ 
J182901.32+002933.0   &  892 (6)  &  0.36 (0.01)   &  -0.54 (0.05)  &  0.23 (0.02)   &  Ser-Bolo 13$^{*}$  &   \\ 
J182901.68+002954.6   &  1158 (3)  &  1.80 (0.01)  &  -1.04 (0.05)  &  0.23 (0.02)   &  Ser-Bolo 13$^{*}$  & CoKu Ser~G3 (4)   \\ 
J182901.68+002946.5   &  1212 (5)  &  0.70 (0.01)  &  -0.65 (0.05)  &  0.25 (0.02)  &  Ser-Bolo 13$^{*}$  & CoKu Ser~G4 (4)    \\ 
\hline
\multicolumn{7}{c}{Ophiuchus}  \\
\hline
J163151.96-245615.7   &  690 (71)  &  1.2 (0.3)  &  -0.17 (0.05) & 0.05 (0.01) &  \ \ \ \ \ \ \ \ \ \ \ \ \ \ $^{*}$ &  \\ 
%J162610.32-242054.6   &  773 (20)  &  0.36 (0.01)  &  -0.46 (0.05) & 0.39 (0.03)  &  Oph-Bolo 4$^{*}$  &  \\ 
J162658.56-244531.6   &  824 (14)  &  1.3 (0.1)  &  -0.45 (0.05) & 0.03 (0.01)  &     &  GY 186 (5)\\ 
J162624.00-241613.4   &  958 (35)  &  1.9 (0.2)  &  -0.71 (0.05) & 0.04 (0.01)  &     &  \\ 
J163945.36-240203.8   &  970 (30)  &  0.84 (0.09)  &  -0.73 (0.05) & 0.03 (0.01)  &     &  \\ 
J162623.28-242100.7   &  1080 (100)  &  2.0 (0.4)  & -0.62 (0.05) & 0.15 (0.01)  &  Oph-Bolo 7$^{*}$  &  GY 20 (5)
\enddata
\tablenotetext{a}{The 1.1~mm mass ($\mathrm{M_{1mm}}$) is calculated for an optically thin disk and a dust temperature of $T_D = 15$~K.  Our assumption for the dust opacity may be incorrect for typical Class~II disks, however, where grain growth is a possibility \citep[e.g.,][]{natta07}.}
\tablenotetext{b}{Bolocam IDs with "*"s indicate that the source is in a confused region at 1.1~mm, and the association of the Spitzer object with the given 1.1~mm emission is not secure.}
\tablenotetext{c}{Typically classified as a Class~I source, RNO~15 has a bolometric temperature just above the Class~I cutoff in our sample.  The spectral index of RNO~15 is $\alpha_{IR} = -0.09$, placing it in the ``flat spectrum'' category, or close to the Class~I boundary.}
\tablecomments{References: (2) \citealt{hk72}; (3) \citealt{asr94}; (4) \citealt{ck79}; (5) \citealt{gy92}.}
\end{deluxetable*}
\endinput

